Representation Learning of Limit Order Book: A Comprehensive Study and Benchmarking

The Limit Order Book (LOB), the mostly fundamental data of the financial market, provides a fine-grained view of market dynamics while poses significant challenges in dealing with the esteemed deep models due to its strong autocorrelation, cross-feature constrains, and feature scale disparity. Existing approaches often tightly couple representation learning with specific downstream tasks in an end-to-end manner, failed to analyze the learned representations individually and explicitly, limiting their reusability and generalization. This paper conducts the first systematic comparative study of LOB representation learning, aiming to identify the effective way of extracting transferable, compact features that capture essential LOB properties. We introduce LOBench, a standardized benchmark with real China A-share market data, offering curated datasets, unified preprocessing, consistent evaluation metrics, and strong baselines. Extensive experiments validate the sufficiency and necessity of LOB representations for various downstream tasks and highlight their advantages over both the traditional task-specific end-to-end models and the advanced representation learning models for general time series. Our work establishes a reproducible framework and provides clear guidelines for future research. Datasets and code will be publicly available at https://github.com/financial-simulation-lab/LOBench.

==> figures/introduction/pipeline.tex <==
\begin{figure*}[!ht]
    \centering
    \begin{tikzpicture}[node distance=2cm]
    
    % Raw Multivariate Time Series
    \node[box] (raw) {Raw Multivariate \\ Time Series};
    
    % Representation Learning
    \node[box, right=4cm of raw] (learning) {Representation \\ Learning};
    
    % Latent Features
    \node[box, right=4cm of learning] (latent) {Latent \\ Features};
    
    % Solvers
    \node[box, right=4cm of latent] (solvers) {Solvers};
    
    % Downstream Tasks
    \node[draw, text centered, thick, minimum width=4cm, minimum height=5cm, right=4cm of solvers] (tasks) {Downstream \\ Tasks};
    
    % Task Boxes inside the Downstream Tasks Box
    \node[draw, text centered, below=0.5cm of tasks.north, yshift=-1.0cm, minimum width=3.5cm, rounded corners] (task1) {Prediction};
    \node[draw, text centered, below=0.7cm of task1, minimum width=3.5cm, rounded corners] (task2) {Classification};
    \node[draw, text centered, below=0.7cm of task2, minimum width=3.5cm, rounded corners] (task3) {Anomaly Detection};
    \node[draw, text centered, below=0.7cm of task3, minimum width=3.5cm, rounded corners] (task4) {Interpolation};
    
    % Arrows connecting boxes
    \draw[arrow] (raw.east) -- (learning.west);
    \draw[arrow] (learning.east) -- (latent.west);
    \draw[arrow] (latent.east) -- (solvers.west);
    \draw[arrow] (solvers.east) -- (tasks.west);
    
    \end{tikzpicture}
    \caption{The basic pipeline of representation learning for MTS.}
    \label{fig:pipeline}
\end{figure*}
